The Inside-out Growth of the Galactic Disk

We quantify the inside-out growth of the Milky Way's low-alpha stellar disk, modelling the ages, metallicities and Galactocentric radii of APOGEE red clump stars with 6 < R < 13 kpc. The current stellar distribution differs significantly from that expected from the star formation history due to the redistribution of stars through radial orbit mixing. We propose and fit a global model for the Milky Way disk, specified by an inside-out star formation history, radial orbit mixing, and an empirical, parametric model for its chemical evolution. We account for the spatially complex survey selection function, and find that the model fits all data well. We find distinct inside-out growth of the Milky Way disk; the best fit model implies that the half-mass radius of the Milky Way disk has grown by 43\% over the last 7 Gyr. Yet, such inside-out growth still results in present-day age gradient weaker than 0.1 Gyr/kpc. Our model predicts the half-mass and half-light sizes of the Galactic disk at earlier epochs, which can be compared to the observed redshift -size relations of disk galaxies. We show that radial orbit migration can reconcile the distinct disk-size evolution with redshift, also expected from cosmological simulations, with the modest present-day age gradients seen in the Milky Way and other galaxies.

==> table_ages.tex <==
%---------------------------------------------------------
% summary table of ages datasets


\begin{table*}
\centering
\caption{\label{table_model_description}Age catalogs summary}
\begin{tabular}{lllll}
\hline

%--------------------------------------
% First row: names of the five columns
%--------------------------------------
%\adjustbox{valign=t}{\makecell[l]{Dataset}}
%& \adjustbox{valign=t}{\makecell[l]{Ness16}}
%&\adjustbox{valign=t}{\makecell[l]{Ness18}}
%&\adjustbox{valign=t}{\makecell{Ting18}} 
%&\adjustbox{valign=t}{\makecell[r]{Sanders18}} \\
Dataset & Ness16 & Ness18 & Ting18 & Sanders18\\

\hline
%-------------------------------------
% Second row: Method
%-------------------------------------
Method & Cannon & Cannon & ANN & ANN + PARSEC \\

%-------------------------------------
% Second.5 row: Complexity
%-------------------------------------
Complexity & Quadratic model & Quadratic model 
& \makecell[l]{150 neurons \\ 3 hidden layers} & \makecell{48 neurons \\ 2 hidden layers} \\

%& \adjustbox{valign=t}{\makecell[l]{150 neurons \\  3 hidden layers}}    
%&\adjustbox{valign=t}{\makecell[l]{48 neurons \\  2 hidden layers}}     \\


%-------------------------------------
% Third row: Training set
%-------------------------------------
\hline
Training set &\adjustbox{valign=t}{\makecell[l]{APOGEE DR12 \\ x APOKASC1 Giants}} 
&  \adjustbox{valign=t}{\makecell[l]{APOGEE DR14 \\ x APOKASC2 Giants}}
&  \adjustbox{valign=t}{\makecell[l]{APOGEE DR14 \\ x APOKASC2 RC}}
& \adjustbox{valign=t}{\makecell[l]{APOGEE DR14 \\ x (Vrard16 $\cup$ APOKASC1) }} \\


%------------------------------------
% Training set size
%------------------------------------
\adjustbox{valign=t}{\makecell[l]{Training set size }}
&\adjustbox{valign=t}{\makecell[l]{1639}} & xxx & 2000 & xxx \\


%-----------------------------------
% Fifth row: Training features
%-----------------------------------
\adjustbox{valign=t}{\makecell[l]{Training features}}
& \adjustbox{valign=t}{\makecell[l]{$F_\lambda$}}
& \adjustbox{valign=t}{\makecell[l]{$F_\lambda$}}
& \adjustbox{valign=t}{\makecell[l]{$F_\lambda$}}
& \adjustbox{valign=t}{\makecell[l]{[M/H], [N/M], [C/M], [O/M] Teff, logg}}\\

%-----------------------------------
% Sixth row: Training labels
%-----------------------------------
\adjustbox{valign=t}{\makecell[l]{Training labels}}
& \adjustbox{valign=t}{\makecell[l]{Log current Mass $M$}}
& \adjustbox{valign=t}{\makecell[l]{Log current Mass $M$}}
& \adjustbox{valign=t}{\makecell[l]{Log age $\tau$}}
& \adjustbox{valign=t}{\makecell[l]{Log current Mass $M$}}\\

%-----------------------------------
% Sixth row: Training set uncertainty on the labels
%-----------------------------------
\adjustbox{valign=t}{\makecell[l]{Uncertainty \\ of the training set \\ on the labels}}
& \adjustbox{valign=t}{\makecell[l]{???}}
& \adjustbox{valign=t}{\makecell[l]{???}}
& \adjustbox{valign=t}{\makecell[l]{?}}
& \adjustbox{valign=t}{\makecell[l]{?}}\\

%-----------------------------------
% Seventh row: Mass loss prescription
%-----------------------------------
\hline
\adjustbox{valign=t}{\makecell[l]{Mass loss \\ prescription}}
& \adjustbox{valign=t}{\makecell[l]{ $\eta_\mathrm{Reimers} = 0.2$}}
& \adjustbox{valign=t}{\makecell[l]{$\eta_\mathrm{Reimers} = 0.2$}}
& \adjustbox{valign=t}{\makecell[l]{Not known}}
& \adjustbox{valign=t}{\makecell[l]{$\eta_\mathrm{Reimers} = 0.2$}}\\

%-----------------------------------
% Eighth row: Testing rms
%-----------------------------------
\hline
\adjustbox{valign=t}{\makecell[l]{Rms on test set}}
& \adjustbox{valign=t}{\makecell[l]{ 0.2 dex in $\log_{10}$ Age}}
& \adjustbox{valign=t}{\makecell[l]{ ??? }}
& \adjustbox{valign=t}{\makecell[l]{0.15 dex in $\log_{10}$ Age}}
& \adjustbox{valign=t}{\makecell[l]{0.15 dex in $\log_{10}$ Age}}\\


\hline
\end{tabular}
\end{table*}


  \begin{center}
    \begin{tabular}{ | c | c | c |}
      \hline
      \thead{A Head} & \thead{A Second \\ Head} & \thead{A Third \\ Head} \\
      \hline
      Some text &  \makecell{Some really \\ longer text}  & Text text text  \\
      \hline
    \end{tabular}
  \end{center}
